A comprehensive evaluation of ChatGPT's zero-shot Text-to-SQL capability

This paper presents the first comprehensive analysis of ChatGPT's Text-to-SQL ability. Given the recent emergence of large-scale conversational language model ChatGPT and its impressive capabilities in both conversational abilities and code generation, we sought to evaluate its Text-to-SQL performance. We conducted experiments on 12 benchmark datasets with different languages, settings, or scenarios, and the results demonstrate that ChatGPT has strong text-to-SQL abilities. Although there is still a gap from the current state-of-the-art (SOTA) model performance, considering that the experiment was conducted in a zero-shot scenario, ChatGPT's performance is still impressive. Notably, in the ADVETA (RPL) scenario, the zero-shot ChatGPT even outperforms the SOTA model that requires fine-tuning on the Spider dataset by 4.1\%, demonstrating its potential for use in practical applications. To support further research in related fields, we have made the data generated by ChatGPT publicly available at https://github.com/THU-BPM/chatgpt-sql.

==> subfiles/999_others.tex <==

\section{Introduction}

These instructions are for authors submitting papers to ACL 2023 using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} as well as guidelines set forth in the ACL 2023 call for papers.\footnote{\url{https://2023.aclweb.org/calls/main_conference/}} This document contains additional instructions for the \LaTeX{} style files.
The templates include the \LaTeX{} source of this document (\texttt{acl2023.tex}),
the \LaTeX{} style file used to format it (\texttt{acl2023.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}
\section{Preamble}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}
The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}
To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{ACL2023}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{ACL2023}
\end{verbatim}
\end{quote}
To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)
Please see the \LaTeX{} source of this document for comments on other packages that may be useful.
Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.
By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}



Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,augenstein-etal-2016-stance,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}
You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}
Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Limitations}
ACL 2023 requires all submissions to have a section titled ``Limitations'', for discussing the limitations of the paper as a complement to the discussion of strengths in the main text. This section should occur after the conclusion, but before the references. It will not count towards the page limit.
The discussion of limitations is mandatory. Papers without a limitation section will be desk-rejected without review.

While we are open to different types of limitations, just mentioning that a set of results have been shown for English only probably does not reflect what we expect. 
Mentioning that the method works mostly for languages with limited morphology, like English, is a much better alternative.
In addition, limitations such as low scalability to long text, the requirement of large GPU resources, or other things that inspire crucial further investigation are welcome.

\section*{Ethics Statement}
Scientific work published at ACL 2023 must comply with the ACL Ethics Policy.\footnote{\url{https://www.aclweb.org/portal/content/acl-code-ethics}} We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).

\section*{Acknowledgements}
This document has been adapted by Jordan Boyd-Graber, Naoaki Okazaki, Anna Rogers from the style files used for earlier ACL, EMNLP and NAACL proceedings, including those for
EACL 2023 by Isabelle Augenstein and Andreas Vlachos,
EMNLP 2022 by Yue Zhang, Ryan Cotterell and Lea Frermann,
ACL 2020 by Steven Bethard, Ryan Cotterell and Rui Yan,
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% Entries for the entire Anthology, followed by custom entries


\appendix

\section{Example Appendix}
\label{sec:appendix}

This is a section in the appendix.

==> tbls/cg-component.tex <==
\begin{table}[bt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{SQL Components} & \textbf{DEV} & \textbf{Non-CG} & \textbf{CG}\\
\midrule 
SELECT & 84.6 & 88.2 & 60.2\\
SELECT (no AGG)   & 86.3 & 89.3 & 62.9\\
WHERE & 80.6 & 91.8 & 62.5\\
WHERE(no OP) & 85.1 & 95.3 & 69.2 \\
GROUP BY (no HAVING)   & 81.1 & 85.7 & 66.4\\
GROUP BY & 76.9 & 81.6 & 54.5 \\
ORDER BY  & 78.2 & 82.0 & 58.3 \\
AND/OR & 99.0 & 99.3 & 91.2\\
KEYWORDS & 86.3 & 92.8 & 67.1 \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy on the different SQL components. The reported results are the average results over \textsc{STaR} and RASAT on three benchmarks of \textsc{SParC}. } 
\label{tab:component}
\vspace{-0.1in}
\end{table}

==> tbls/cosql-cg.tex <==
\begin{table}[bt!]
\centering
\resizebox{0.97\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Methods} & \textbf{Dev} & \textbf{Non-CG} & \textbf{CG}\\
\midrule 
SPIC (concat) + BERT-large & - & - & -\\
SPIC (turn) + BERT-large  & - & - & -\\
SPIC (gate) + BERT-large  & - & - & -\\
RAT-SQL + \textsc{SCoRe}  & - & - & -\\
LGESQL + ELECTRA-large & - & - & - \\
LGESQL + \textsc{STaR} & - & - & - \\
PICARD + T5-3B & - & - & -\\
RASAT  + T5-3B & - & - & - \\
\bottomrule
\end{tabular}}
\vspace{-2mm}
\caption{Results on \textsc{CoSQL}}
\label{tab:token}
% \vspace{-0.1in}
\end{table}

==> tbls/dataset_sta.tex <==
% \begin{table}[bt!]
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
%  & \textbf{\textsc{SParC}} & \textbf{\textsc{SParC-CG}} & \textbf{\textsc{CoSQL}} & \textbf{\textsc{CoSQL-CG}} \\
% \midrule 
% \# Dialogs  & 422 & 372 & 293 & 167\\
% \# Questions & 1625 & 922 & 1300 & 471 \\
% \# Non-CG Questions & 491 & 491 & 207 & 207\\
% \# CG Questions  & 31 & 431 & 14 & 264\\
% Avg \# Q./Dialog  & 3.85 & 2.47 & 4.44 & 2.82\\
% \bottomrule
% \end{tabular}}
% \caption{The detailed statistics of \textsc{SParC-CG} and  \textsc{CoSQL-CG} benchmark.}
% \label{tab:token}
% % \vspace{-0.1in}
% \end{table}


\begin{table}[bt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
 & \# Questions & \# Non-CG Questions & \# CG Questions \\
\midrule 
\textbf{\textsc{SParC}} & 1625 & 491 & 31 \\
\textbf{\textsc{SParC-CG}} & 863 & 491 & \textbf{372} \\
\textbf{\textsc{CoSQL}}   & 1300 & 207 & 14\\
\textbf{\textsc{CoSQL-CG}} & 474 & 207 & \textbf{267}\\
\bottomrule
\end{tabular}}
\caption{The detailed statistics of \textsc{SParC-CG} and  \textsc{CoSQL-CG} benchmark.}
\label{tab:sta}
% \vspace{-0.1in}
\end{table}


==> tbls/error.tex <==
\begin{table}[bt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Error component} & \textbf{\textsc{STaR}} & \textbf{\textsc{RASAT}} & \textbf{LGESQL}\\
\midrule 
Context Info & 24 & 15 & 25\\
Modification Info   & 149 & 136 & 139\\
Context \& Modification Info  & 112 & 128 & 127\\
\bottomrule
\end{tabular}}
% \vspace{-2mm}
\caption{Statistical analysis of different error types on \textsc{SParC-CG} benchmark.}
\label{tab:err}
\vspace{-0.1in}
\end{table}

==> tbls/main.tex <==
\begin{table*}[bt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Methods / Datasets}}  & \multicolumn{3}{c}{\textsc{SParC}} & \multicolumn{3}{c}{\textsc{CoSQL}}  \\
\cmidrule(lr){2-4}  \cmidrule(lr){5-7} 
& \textbf{Dev} & \textbf{Non-CG} & \textbf{CG} & \textbf{Dev} & \textbf{Non-CG} & \textbf{CG}\\ 
\midrule 
\textsc{SPiC} (\textsc{Concat}) + BERT-Large \cite{DBLP:conf/ijcai/LiuCGLZZ20} & 55.3 & 63.4 & 18.9(36.4$\downarrow$) & 45.2 & 52.3 & 13.3(31.9$\downarrow$)\\
\textsc{SPiC} (\textsc{Turn}) + BERT-Large \cite{DBLP:conf/ijcai/LiuCGLZZ20} & 54.6 & 62.1 & 18.2(36.4$\downarrow$)  & 44.8 & 51.3 & 12.2(32.6$\downarrow$)\\
\textsc{SPiC} (\textsc{Gate}) + BERT-Large  \cite{DBLP:conf/ijcai/LiuCGLZZ20} & 54.3 & 62.4 & 17.3(37.0$\downarrow$)  & 44.2 & 51.8 & 12.4(31.8$\downarrow$)\\
RAT-SQL + \textsc{SCoRe} \cite{DBLP:conf/iclr/0009ZPMA21} & 60.4 & 69.6 & 20.4(40.0$\downarrow$) & 52.1 & 55.6 & 20.4(31.7$\downarrow$)\\
LGESQL + ELECTRA-Large \cite{DBLP:conf/acl/CaoC0ZZ020}& 65.0 & 73.4 & 23.2(41.8$\downarrow$) & 54.4 & 62.4 & 20.4(34.0$\downarrow$) \\
LGESQL + \textsc{STaR} \cite{cai2022star} & 66.9 & 75.4 & 23.4(43.5$\downarrow$)  & 59.7 & 68.4 & 25.1(34.6$\downarrow$) \\
PICARD + T5-3B \cite{scholak-etal-2021-picard}  & - & - & - & 56.9 & 58.1 & 21.5(35.4$\downarrow$) \\
RASAT  + T5-3B \cite{DBLP:journals/corr/abs-2205-06983}  & 66.7 & 75.8 & 22.0(44.7$\downarrow$)  & 58.8 & 67.9 & 20.4(38.4$\downarrow$) \\
\bottomrule
\end{tabular}}
% \vspace{-2mm}
\caption{Question match accuracy of current competitive models on three different benchmarks: Dev, Non-CG, and CG. For all the models, we adopt the given parameters. }
\label{tab:main}
\vspace{-0.1in}
\end{table*}

==> tbls/palign.tex <==
\begin{table}[bt!]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|ccc}
\toprule
\multicolumn{1}{c}{\textbf{Methods}} & \multicolumn{1}{c}{\textbf{DEV}} & \multicolumn{1}{c}{\textbf{Non-CG}} & \multicolumn{1}{c}{\textbf{CG}} 
% \textbf{Methods} & \textbf{Dev QM} & \textbf{Non-CG} & \textbf{CG}
\\
\midrule 
\multicolumn{4}{c}{\textsc{SParC}} \\
\midrule
\textsc{SPiC} (\textsc{Concat}) + BERT-Base & 47.6 & 53.5 & 8.6\\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}  & 50.6 & 54.1& 14.8(6.2$\uparrow$) \\
\textsc{SPiC} (\textsc{Concat}) + BERT-Large  & 55.3 & 63.4 & 18.9\\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}  & 56.1 & 63.8 & 20.1(1.2$\uparrow$)\\
LGESQL + ELECTRA-Large & 65.0 & 73.4 & 23.2 \\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}   & 64.8 & 73.0 & 25.3(2.1$\uparrow$) \\
 \midrule 
\multicolumn{4}{c}{\textsc{CoSQL}} \\
\midrule
\textsc{SPiC} (\textsc{Concat}) + BERT-Base  & 39.2 & 35.0  &  5.2\\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}   & 40.5 & 36.2 & 9.6(4.4$\uparrow$)\\
\textsc{SPiC} (\textsc{Concat}) + BERT-Large  & 45.2 & 52.3 & 12.2\\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}   & 45.5 & 52.7& 14.4(2.2$\uparrow$)\\
LGESQL + ELECTRA-Large  & 54.4 & 62.4 & 20.4 \\
 \quad \quad \quad \quad \quad \quad w. \texttt{p-align}  & 53.8 & 62.3& 21.2(0.8$\uparrow$)\\
 \midrule
\bottomrule
\end{tabular}}
% \vspace{-2mm}
\caption{The results of different models w. \& w/o \texttt{p-align} on three benchmarks of \textsc{SParC} and \textsc{CoSQL}.}
\label{tab:palign}
\vspace{-0.1in}
\end{table}
